MetaCOG: A Hierarchical Probabilistic Model for Learning Meta-Cognitive Visual Representations

Humans have the capacity to question what we see and to recognize when our vision is unreliable (e.g., when we realize that we are experiencing a visual illusion). Inspired by this capacity, we present MetaCOG: a hierarchical probabilistic model that can be attached to a neural object detector to monitor its outputs and determine their reliability. MetaCOG achieves this by learning a probabilistic model of the object detector's performance via Bayesian inference -- i.e., a meta-cognitive representation of the network's propensity to hallucinate or miss different object categories. Given a set of video frames processed by an object detector, MetaCOG performs joint inference over the underlying 3D scene and the detector's performance, grounding inference on a basic assumption of object permanence. Paired with three neural object detectors, we show that MetaCOG accurately recovers each detector's performance parameters and improves the overall system's accuracy. We additionally show that MetaCOG is robust to varying levels of error in object detector outputs, showing proof-of-concept for a novel approach to the problem of detecting and correcting errors in vision systems when ground-truth is not available.

==> Old_and_scrap_versions/scrap_text.tex <==
%There are two main insights that we draw upon. First, human vision is an encapsulated black-box system and we do not have access to its internal computations \citep{firestone2016cognition}. Yet, people are still able to learn a model of their own visual system \citep{berkeBBS}. This is proof-of-concept that such learning is possible, and we therefore focus on a problem formulation where the meta-cognitive system does not have access to the internal architecture of the object detector---only its outputs. Second, people can detect failures in their visual system spontaneously and without feedback or access to ground-truth \citep{berkeBBS}, so we therefore aim to do the same in our model by drawing on insights about how humans represent themselves and the objects around them: Humans embed both their own body and object detections in three-dimensional representations \citep{spelke2023precis}. These representations assume object permanence (i.e., objects in the world continue to exist even when they cannot be seen; \citet{carey2009origin}; \citet{spelke2007core}) and access to our own viewpoint (i.e., we know when we turn our head and how our viewpoint changes as we move through space). For instance, if you detect an object in your periphery but it disappears when you turn your head to look directly at it, you can conclude your visual system made an error, because objects do not spontaneously teleport or cease to exist.
